Stackelberg Equilibria for Two-Player Network Routing Games on Parallel Networks

We consider a two-player zero-sum network routing game in which a router wants to maximize the amount of legitimate traffic that flows from a given source node to a destination node and an attacker wants to block as much legitimate traffic as possible by flooding the network with malicious traffic. We address scenarios with asymmetric information, in which the router must reveal its policy before the attacker decides how to distribute the malicious traffic among the network links, which is naturally modeled by the notion of Stackelberg equilibria. The paper focuses on parallel networks, and includes three main contributions: we show that computing the optimal attack policy against a given routing policy is an NP-hard problem; we establish conditions under which the Stackelberg equilibria lead to no regret; and we provide a metric that can be used to quantify how uncertainty about the attacker's capabilities limits the router's performance.

==> src/equilibria2.tex <==
\section{Equilibria} \label{sec:equilibria}

In this section, we present results that describe precisely the relationship between SE and NE in our model. For some $E' \subseteq E$, we denote it's total capacity as $C(E') := \sum_{e \in E'} c_e$. 

\begin{theorem} \label{thm:equilibria}
	For a parallel network, $\mathcal{N}(r, r^a)$ is nonempty if and only if one of the following conditions is satisfied:
	\begin{align}
	    &r^a \leq \max_{E' \subseteq E}\frac{C(E') - r}{|E'|} \label{eq:low_a} \\ 
		&r^a \geq C(E) - \max_{E' \subseteq E}\frac{r - C(E\setminus E')}{|E'|}. \label{eq:high_a}
    \end{align}
	Furthermore, if either \eqref{eq:low_a} or \eqref{eq:high_a} holds, then $\mathcal{N}(r, r^a) = \mathcal{S}(r, r^a)$. \footnote{While finding the maxima in \eqref{eq:low_a} and \eqref{eq:high_a} may appear to be computationally intractable given the number of edges in the network, there exist linear-time algorithms that can compute each. The presentation of these algorithms is outside the scope of this work, however.}
\end{theorem}

The proof can be found in Appendix\ref{sec:proof_eqilibria}. The intuition behind this theorem is that $(f, f^a)$ cannot be a NE if there are two edges $d,e$ such that $B_d(f, f^a) = f_d+f^a_d-c_d > 0$ and $f_e + f_e^a - c_e < 0$. Under these conditions, the router is unilaterally incentivized to reroute some traffic from $d$ to $e$. Thus the two extremes in Theorem \ref{thm:equilibria}: the condition in \eqref{eq:low_a}, where the attacker does not have enough power to block any routed traffic, and the condition \eqref{eq:high_a}, where such an $e$ cannot exist. If the attack power $r^a$ is anywhere in between the two extremes, then the router will always have a unilateral incentive to change its route. This phenomenon is illustrated in Figure \ref{fig:se_v_ne}.

The following corollary is shown as part of the proof for Theorem \ref{thm:equilibria}:

\begin{cor} \label{cor:eqpolicies}
    For a parallel network, if \eqref{eq:low_a} is satisfied, then a SE and NE routing policy is
    \begin{equation} \label{eq:low_a_rt}
		f_e = f^{\rm lo}_e := \max\left\{c_e - \max_{E' \subseteq E}\frac{C(E') - r}{|E'|}, 0\right\},
	\end{equation}
	where $B(f^{\rm lo}, f^a) = 0$ for any $f^a \in \mathcal{F}^a(c, r^a)$.
	If \eqref{eq:high_a} is satisfied, then a SE and NE routing policy is
	\begin{equation} \label{eq:high_a_rt}
		f_e = f^{\rm hi}_e := \min\left\{c_e, \max_{E' \subseteq E}\frac{r - C(E\setminus E')}{|E'|}\right\}, 
	\end{equation}
	where $B(f^{\rm hi}, f^a) = r + r^a - C(E)$ for any $f^a \in \mathcal{F}^a(c, r^a)$.
\end{cor}

For notational purposes, we define
\begin{align}
    g :=& \max_{E' \subseteq E} \frac{C(E') - r}{|E'|}\\
    h :=& \max_{E' \subseteq E} \frac{r - C(E \setminus E'))}{|E'|}.
\end{align}
Refer again to the network in Figure \ref{fig:ex_model}. At point $P_!$, $r=20$ and $r^a=5$. Here we calculate $g = 7$, which means when $r^a \leq g$, satisfying the condition in \eqref{eq:low_a}. Thus the router can use the policy $f = \{0, 0, 2, 5, 13\}$ to ensure that the attacker cannot block any traffic. By Theorem \ref{thm:equilibria}, this also implies that $(f, f^a)$ is both a SE and a NE for any $f^a \in \mathcal{F}^a(c, r)$. At point $P_3$, $r=25$ and $r^a = 45$. Here we calculate $h = 19/3 = 6.\bar{3}$ and $C(E) = 47$, which means that $r_a \geq C(E) - h$. Thus the router can use the policy $f = \{2, 4, 6.\bar{3}, 6.\bar{3}, 6.\bar{3}\}$, and from Theorem \ref{thm:equilibria}, $(f, f^a)$ is a NE and SE for any $f^a \in \mathcal{F}^a(c, r)$. At point $P_2$, $r=30$ and $r^a=20$. We calculate $g = 3.75$ and $h = 8$. Since $g < r^a < C(E) - h$, we know that no NE can exist at this point.
